Streaming Algorithms for Stochastic Multi-armed Bandits

We study the Stochastic Multi-armed Bandit problem under bounded arm-memory. In this setting, the arms arrive in a stream, and the number of arms that can be stored in the memory at any time, is bounded. The decision-maker can only pull arms that are present in the memory. We address the problem from the perspective of two standard objectives: 1) regret minimization, and 2) best-arm identification. For regret minimization, we settle an important open question by showing an almost tight hardness. We show {\Omega}(T^{2/3}) cumulative regret in expectation for arm-memory size of (n-1), where n is the number of arms. For best-arm identification, we study two algorithms. First, we present an O(r) arm-memory r-round adaptive streaming algorithm to find an {\epsilon}-best arm. In r-round adaptive streaming algorithm for best-arm identification, the arm pulls in each round are decided based on the observed outcomes in the earlier rounds. The best-arm is the output at the end of r rounds. The upper bound on the sample complexity of our algorithm matches with the lower bound for any r-round adaptive streaming algorithm. Secondly, we present a heuristic to find the {\epsilon}-best arm with optimal sample complexity, by storing only one extra arm in the memory.

==> section_proposedFix.tex <==
\section{Proposed Algorithm}
\label{section:fix}
We propose an $(\varepsilon, \delta)$-PAC algorithm (Algorithm \ref{algo:AssadiFixed}) for the \SMAB problem having the optimal sample complexity $O(\frac{n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta}))$ and which uses $O(\log^* n)$ space. Before formally bounding the sample complexity and proving the correctness of our algorithm, we provide intuition for why our algorithm works while that of \cite{ASSADI2020} does not, especially since the two algorithms differ in a single step (Line 12 in both Algorithm \ref{algo:AssadiOriginal} and Algorithm \ref{algo:AssadiFixed}).

Consider any level $\ell$, and an arm $arm'$ that reaches level $\ell$. Once $arm'$ reaches level $\ell$, our algorithm pulls $arm'$ $s_\ell$ number of times and compares its empirical mean with that of $arm^*_\ell$, the current best arm at level $\ell$. If $arm'$ loses to $arm^*_\ell$, then we discard $arm'$ and move to the next arm in the stream. On the other hand, if $arm'$ wins against $arm^*_\ell$ then we replace the current $arm^*_\ell$ with $arm'$. Additionally, and unlike in \cite{ASSADI2020}, we store the empirical mean of $arm'$ for future challenges. The arm, $arm'$, is not be pulled in level $\ell$ again. Once the counter $C_\ell$ reaches $c_\ell$, we send $arm^*_\ell$ to level $\ell+1$.

%Our algorithm with space constraints can be interpreted as the following algorithm which does not have space constraints. 
An equivalent algorithm, but one without space constraints, is the one which simultaneously pulls each of the $c_\ell$ arms $s_\ell$ number of times and sends the arm with the highest empirical means to level $\ell+1$. In this case, we can bound by a very small value the probability that an arm with a reward-gap $> \varepsilon_\ell$ from the best arm among the $c_\ell$ arms defeats the best arm. Thus, storing not just the arm with the highest empirical mean seen so far, but also the empirical mean itself, enables us to use the history and ensure the correctness of the algorithm.

\begin{thm}
	\label{theorem:fix analysis}
	Algorithm \ref{algo:AssadiFixed} is an $(\varepsilon,\delta)$-PAC algorithm with sample complexity $O(\frac{n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta}))$ and space complexity $O(\log^* n)$.
\end{thm}
\begin{proof}
	We prove this theorem using the following lemmas. Lemma \ref{lemma:fix sample complexity} shows that the sample complexity of our algorithm is $O(\frac{n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta}))$. In Lemma \ref{lemma: fix correctness}, we prove the correctness of the algorithm. Further, at each of the $\lceil \log^* n \rceil + 1$ levels we store the empirical mean of a single arm which implies the space complexity of our algorithm.
\end{proof}

\begin{algorithm}[ht!]
\caption{}
\label{algo:AssadiFixed}
\begin{algorithmic}[1]
\STATE $\{r_\ell\}^{\infty}_{\ell=1}:r_1:=4,r_{\ell+1}=2^{r_\ell}$
\STATE $\varepsilon_\ell=\frac{\varepsilon}{10\cdot 2^{\ell-1}}$
\STATE $\beta_\ell=\frac{1}{\varepsilon^2_\ell}$
\STATE $s_\ell = 4\beta_\ell\big(\ln(\frac{1}{\delta}+3r_\ell)\big)$
\STATE $c_1=2^{r_1},$ $c_\ell=\frac{2^{r_\ell}}{2^{\ell-1}}(\ell\geq2)$
\STATE Counters: $C_1,C_2,\ldots,C_t$ initialized to 0 where $t=\lceil \log^*(n)\rceil+1$
\STATE Stored arms: $arm^*_1,arm^*_2,\ldots,arm^*_t$ the most biased arm of $\ell$-th level.
\STATE Stored empirical means: $p^*_1,p^*_2,\ldots,p^*_t$, the highest empirical mean of $\ell$-th level, initialized to 0.
\WHILE {A new arm $arm_i$ arrives in the stream}
\STATE Read $arm_i$ to memory
\STATE \textbf{\underline{Aggressive Selective Promotion:}} Starting from level $\ell$=1:
%\IF{$C_\ell = 0$}\label{st1}
%\STATE Sample $arm_i$ for $s_\ell$ times and store the empirical mean in $p^*_\ell$
%\ELSE
\STATE \label{next level} Sample $arm_i$ for $s_\ell$ times and compare its empirical mean with $p^*_\ell$. 
\STATE Drop $arm_i$ if $\hat{p}_{arm_i} <p^*_\ell$, otherwise replace $arm^*_\ell$ with $arm_i$ and make $p^*_\ell$ equal to $\hat{p}_{arm_i}$
\STATE Increase $C_\ell$ by 1
\STATE If $C_\ell=c_\ell$, make $C_\ell$ equal to 0, send $arm^*_\ell$ to the next level by calling Line \ref{next level} with $(\ell=\ell+1)$
%\ENDIF
\ENDWHILE
\STATE Return $arm^*_t$ as the selected most bias arm  
\end{algorithmic}
\end{algorithm}

Next, we bound the sample complexity of our algorithm.

\begin{lem}
	\label{lemma:fix sample complexity}
	The sample complexity of the algorithm is $O(\frac{n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta}))$.
\end{lem}
\begin{proof}
%In any level $\ell$, Algorithm \ref{algo:AssadiFixed} pulls only the newly arrived arm $s_\ell$ number of times. On the other hand the algorithm in \cite{ASSADI2020} pulls both the newly arrived arm as well as $arm^*_{\ell}$ $s_\ell$ number of times each. Hence, the number of arm pulls in our algorithm is less than that in \cite{ASSADI2020}. Since the total number of arm pulls in \cite{ASSADI2020} is  $O(\frac{n}{\varepsilon^2}\cdot ln(\frac{1}{\delta}))$, the lemma follows.
For any level $\ell-1$, we send one arm from level $\ell-1$ to level $\ell$ for every $c_{\ell-1}$ arms seen. Hence, number of arms that can reach any level $\ell$ is at most $\frac{n}{\prod_{i=1}^{\ell-1}c_i}$. Each arm arriving at level $\ell$ is pulled exactly $s_\ell$ times. Since we have $\ceil{\log^* n} + 1$ levels, the total number of samples can be bounded as:
\begin{align*}
	\sum_{\ell=1}^{\ceil{\log^* n}+1} \frac{n}{\prod_{i=1}^{\ell-1}c_i} \cdot s_\ell & =  \sum_{\ell=1}^{\ceil{\log^* n}+1} \frac{4n\beta_\ell\Big(\ln(\frac{1}{\delta} + 3r_\ell)\Big)}{\prod_{i=1}^{\ell-1}c_i}\\
	& = \frac{4n}{\varepsilon^2} \sum_{\ell=1}^{\ceil{\log^* n} +1} \frac{\Big(\ln(\frac{1}{\delta} + 3r_\ell)\Big)}{\prod_{i=1}^{\ell-1}c_i} \cdot (10\cdot 2^{\ell-1})^2 \tag{\text{From the definition of} $\beta_\ell$}\\
	& \leq \frac{400n}{\varepsilon^2} \sum_{\ell=1}^{\infty} \frac{\ln(\frac{1}{\delta})}{c_{\ell-1}}\cdot 4^{\ell-1} + \frac{3r_\ell}{c_{\ell-1}\cdot c_{\ell-2}} \cdot (2^{\ell-1})^2 \tag{Since $\prod_{i=1}^{\ell-1}c_i \geq c_{\ell-1}\cdot c_{\ell-2} \geq c_{\ell-1}$}\\
	& = \frac{400n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta})\sum_{\ell=1}^{\infty}\frac{2^{3\ell - 4}}{2^{r_{\ell-1}}} + \frac{1200n}{\varepsilon^2}\sum_{\ell=1}^{\infty}\frac{2^{4\ell - 7}}{2^{r_{\ell-2}}}\\
	& \leq \frac{800n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta}) + \frac{1200n}{\varepsilon^2} (O(1) + \sum_{\ell=5}^{\infty}\frac{2^{4\ell - 7}}{2^{r_{\ell-2}}}) \tag{$\sum_{\ell=1}^{4}\frac{2^{4\ell - 7}}{2^{r_{\ell-2}}} = O(1)$}\\
	& \leq \frac{800n}{\varepsilon^2}\cdot \ln(\frac{1}{\delta}) + O(1)\cdot \frac{n}{\varepsilon^2} \tag{Since $\sum_{\ell=5}^{\infty}\frac{2^{4\ell - 7}}{2^{r_{\ell-2}}} < 1$}\\
\end{align*}
Hence, we have that the sample complexity is $O(\frac{n}{\varepsilon^2}\log(1/\delta))$.
\end{proof}

\begin{lem}
	\label{lemma: fix correctness}
	With probability at least $1-\delta$, the arm selected by the algorithm is an $\varepsilon$-best arm.
\end{lem}
\begin{proof}
We prove this lemma using the following claim.
\begin{claim}
	\label{claim:level_suboptimality}
	For any level $\ell$, let $a^*_\ell$ be the best arm to ever reach this level. Then, with probability at least $1 - \frac{\delta}{2^{\ell+1}}$, an arm with reward gap at most $\varepsilon_\ell$ from $a^*_\ell$ is sent to level $\ell + 1$.
\end{claim}	
\begin{proof}
	Let us consider some level $\ell$ and a set of arms $a_1,a_2,\ldots,a_{c_\ell}$ which increase the counter $C_\ell$ from $0$ to $c_\ell$. Denote the best arm among them as $a^*$ and let $arm^*_\ell$ be used to denote the empirically best arm seen so far since the arrival of $a_1$.  Our algorithm works as follows: once an arm arrives at level $\ell$, it is pulled $s_\ell$ number of times. Next, we compare its empirical mean with that of $arm^*_\ell$, which was computed when the arm corresponding to $arm^*_\ell$ arrived at level $\ell$. The arm with the greater empirical mean is maintained as $arm^*_\ell$ and its empirical mean is stored for future comparisons. Once $C_\ell = c_\ell$, $arm^*_\ell$ is sent to level $\ell + 1$. Note that this is equivalent to simultaneously pulling each of the $c_\ell$ arms $s_\ell$ number of times, and then sending the empirically best arm to level $\ell+1$.
	
	Hence, as shown in \cite{ASSADI2020}, at any level $\ell$, if two arms have reward gap $p_i - p_j \geq \varepsilon_\ell$ then $\text{Pr}[\hat{p_i} < \hat{p_j}] \leq \frac{\delta}{2^{r_\ell+2}}$. Since at most $c_\ell$ arms arrive at level $\ell$ before the counter $C_\ell$ reaches $c_\ell$, taking union bound we have that the probability of sending an arm with reward gap $\geq \varepsilon_\ell$ with respect to $a^*$ to level $\ell+1$ is at most $\frac{\delta}{2^{r_\ell+2}}\cdot \frac{2^{r_\ell}}{2^{\ell-1}}=\frac{\delta}{2^{\ell+1}}$.
\end{proof}	

By taking a union bound over all $\lceil \log^* n\rceil + 1$ levels, we bound the probability of sending all arms that are non-$\varepsilon_\ell$-optimal to level $\ell+1$ by:
$$ \sum_{\ell = 1}^{\lceil \log^* n\rceil + 1} \frac{\delta}{2^{\ell+1}} \leq \delta \sum_{\ell=1}^\infty \frac{1}{2^{\ell+1}} = \frac{\delta}{2} \leq \delta$$

%\begin{align*}
%	\sum_{\ell = 1}^{\lceil \log^* n\rceil + 1} \frac{\delta}{2^{\ell+1}} &\leq \delta \sum_{\ell=1}^\infty \frac{1}{2^{\ell+1}}\\
%	& = \frac{\delta}{2}\\
%	& \leq \delta
%\end{align*}

As the arms arrive in a stream, the best arm, $arm^*$, enters at level $1$. As shown in Claim \ref{claim:level_suboptimality}, at any level $\ell$, at least one arm with reward gap $\leq \varepsilon_\ell$ from the best arm to arrive at level $\ell$, is sent to level $\ell + 1$. This implies that with probability at least $1- \sum_{i=1}^{\ell-1} \frac{\delta}{2^{\ell+1}}$, at least one arm with reward gap $\leq \sum_{i=1}^{\ell-1}\varepsilon_\ell$ from $arm^*$ arrives at level $\ell$. Summing over the sub-optimality gap accrued over all level, we obtain that with probability at least $1-\delta$, an arm with gap at most:

$$\sum_{\ell = 1}^{\lceil \log^* n\rceil + 1} \varepsilon_\ell = \sum_{\ell = 1}^{\lceil \log^* n\rceil + 1} \frac{\varepsilon}{10 \cdot 2^{\ell - 1}} \leq \frac{\varepsilon}{10}\sum_{\ell = 1}^\infty \frac{1}{2^{\ell - 1}} \leq \varepsilon$$

%\begin{align*}
%	\sum_{\ell = 1}^{\lceil \log^* n\rceil + 1} \varepsilon_\ell & = \sum_{\ell = 1}^{\lceil \log^* n\rceil + 1} \frac{\varepsilon}{10 \cdot 2^{\ell - 1}}\\
%	& \leq \frac{\varepsilon}{10}\sum_{\ell = 1}^\infty \frac{1}{2^{\ell - 1}}\\
%	& \leq \varepsilon
%\end{align*} 

\noindent is output by the algorithm. This concludes the proof of this lemma.

\arn{Note that we can modify the algorithm in this section appropriately so that by storing $r\leq log^*(n)$ coins we can find the $\varepsilon$-best coin with probability atleast $(1-\delta)$ and the sample complexity is $O(\frac{n}{\varepsilon^2}ilog^{(r)}(n))$}
\end{proof}

==> section_regretLowerBound_copy.tex <==
\section{Regret Minimization (Copy Version)}
In the previous sections, we focused on the \emph{pure-exploration} variant of \MAB where the goal is to identify the best arm in terms of its expected reward. We now focus on the \emph{regret minimization} problem in the \MAB problem which leads to the \emph{explore vs. exploit dilemma}. Let us consider an instance of the \SMAB problem with $n$ arms, where arm $i$ has expected reward $\mu_i$. We denote by $\mu^*$ the optimal (aka best) arm in the set of arms, i.e., $\mu^* = \max_{i \in [m]} \mu_i$. Then, the cumulative regret of an algorithm after $T$ rounds is defined as follows:
\begin{definition}[Cumulative Regret]
	Given an instance of the \SMAB problem with $n$ arms, where arm $i$ has expected reward $\mu_i$, the cumulative regret of an algorithm after $T$ rounds is defined as
	\begin{equation}
		R(T) = \mu^*\cdot T - \sum_{t=1}^T \mu_{i_t}
	\end{equation}
	where $i_t$ is the arm pulled by the algorithm at time $t \in [T]$.
\end{definition}
The expected cumulative regret of an algorithm is defined as $\mathbb{E}[R(T)] = \mu^*\cdot T - \sum_{t=1}^T\mathbb{E}[\mu_{i_t}]$, where the expectation is over the randomness in the algorithm and the distribution of rewards.

Recent works by \cite{CHAUDHURI2019} and \cite{LIAU2018} study the problem of regret minimization in the \MAB setting with constraints on the number of arms that can be stored in memory at any time. The algorithms in both these works achieve sub-linear regret (see Section \ref{section:related work} for a detailed discussion) while storing $< n$ arms in memory. Crucially, both these algorithms use multiple passes through the set of arms to achieve their regret guarantees, i.e., they assume that an arm which has been discarded from memory can be read into memory in the future. An interesting direction that remains open is to check if sub-linear regret can be achieved with a single-pass algorithm where an arm, once discarded from memory, cannot to be read into memory again. A question left open in \cite{CHAUDHURI2019} is to provide a lower bound on the expected cumulative regret of an algorithm with bounded memory. We make an important contribution in this direction by showing that any single-pass algorithm for such a setting incurs at least $\Omega(T^{2/3})$ regret.

\begin{thm}
In the \SMAB setting, fix the number of arms $n$ and the time horizon $T$ . For any online \SMAB algorithm, if we are allowed to store at most $m < n$ arms, then there exists a problem instance such that $\mathbb{E}[R(T)] \geq \Omega(\frac{T^{2/3}}{m^{7/3}})$ 
\end{thm}
\begin{proof}
	%\vis{Denote by $M$ the set of indices of arms currently in memory}. 
	We consider $0-1$ rewards and the following two families of problem instances each containing $n$ arms, with parameter $\epsilon>0$ (where $\epsilon=\frac{1}{m^{1/3}T^{1/3}}$.). For each \arn{$j \in [m]$}, let\\
	\begin{align*}
	\mathcal{I}_j^1 = \left\{ \begin{array}{rcl}
	\mu_i & =(1+\epsilon)/2& \mbox{for arm~~}  i=j \\ 
	\mu_i & = 1/2~~~~~~~ &  \mbox{ otherwise}
	\end{array}\right.
	\end{align*}
	
	\begin{align*}
	\mathcal{I}_j^2= \left\{ \begin{array}{rcl}
	\mu_i &= (1+\epsilon)/2 & \mbox{for arm~~} i=j \\ 
	\mu_i &= 1/2~~~~~~~  &\mbox{for~~} i\neq j \text{ and }i\neq n\\
	\mu_i &= 1~~~~~~~~~~ & \mbox{for~~}  i=n
	\end{array}\right.
	\end{align*}

\arn{We also provide one additional problem instance $\mathcal{I}_0'$ containg $n$ arms:
 \begin{align*}
	\mathcal{I}_0'= \left\{ \begin{array}{rcl}
	\mu_i &= 1/2~~~~~~~  &\mbox{for~~} i\neq n\\
	\mu_i &= 1~~~~~~~~~~ & \mbox{for~~}  i=n
	\end{array}\right.
	\end{align*}	}
	\noindent In the above instances, $\mu_i$ denotes the expected reward of the $i^{th}$ arm to arrive in the stream.\\
	
	Note that an algorithm that directly stores the first $m$ arms in the memory will in no way perform worse than any other algorithm that processes the first $m$ arms in some different manner. This is because the processing of any such algorithm can be replicated by an algorithm which directly stores the first $m$ arms. 
	
	Now, when the future arms (arm $m+1$ onward) arrive in the stream, we have to discard at least one of the first $m$ arms from memory in order to store the arriving arms. Note that if we don't discard any arm from the first $m$ arms and instead discard the arriving arms (without processing them at all) then clearly, for all the instances $\mathcal{I}_j^2$ where $j\in[m]$, the algorithm suffers a regret of $\Omega(T)$. Hence, any algorithm that hopes to achieve better regret has to discard at least one of the first $m$ arms from memory. 
	
	
	
	%In each round $t \in [T']$ where $T' \leq T$, the algorithm samples an arm $i$ which is currently in memory and observes a reward $r_s(i)$ where $s$ is the number of times arm $i$ has been sampled till round $t$ and $r_s(i)$ represents the reward of $i$ when we sample it for the $s^{th}$ time.After $T'$ rounds of sampling, suppose that the algorithm decides to discard a set of arms $Y_{T'}$ for the first time. 
	
	%Now, let us define a sample space $\Omega$. 
	We next set up the sample space. Let $L = \frac{1}{4m^2\epsilon^2}$. \vis{Further, let $(r_s(i): i\in[m], s \in [L])$ be a tuple of i.i.d. Bernoulli random variables where $r_s(i)$ has expectation $\mu_i$. We interpret $r_s(i)$ as the reward obtained when arm $i$ is pulled for the $s^{th}$ time and the tuple is called the \emph{rewards table}. The sample space is then expressed as $\Omega = \{0,1\}^{m\times L}$ and any $\omega \in \Omega$ can be interpreted as a realization of the rewards table.}
	%The $L$-round sample space of arm $i$ is then $\Omega_i^L = \{0,1\}^L$, where each outcome corresponds to a particular realization of the tuple $(r_s(i): s \in [L])$. The sample space is then expressed as $\Omega=\Pi_{i\in[m]}\Omega_i^{L}$.\\

\arn{(Definition of $\mathcal{I}_j$ can we change it to set of instances instead of instance. Just check which one is appropriate for formal proof)}
	
	For each $j\in [m]$, let $\mathcal{I}_j$ be an instance such that among the first $m$ incoming arms in the stream, the $j^{th}$ arm has an expected reward $(1+\epsilon)/2$ and rest of the arms have an expected reward $1/2$. 
	
	Each instance $\mathcal{I}_j$ (where $j \in \{1,\ldots, m\}$), defines a distribution $P_j$ on $\Omega$ as follows:
	\begin{equation*}
	\text{P}_j(A)= \mathbb{P}[A~|~\mathcal{I}_j], \text{~~~~~for each $A\subseteq \Omega$}
	\end{equation*}
	\arn{For the instance $\mathcal{I}_0'$, we define a distribution $P_0$ on $\Omega$ as follows:
	\begin{equation*}
	\text{P}_0(A)= \mathbb{P}[A~|~\mathcal{I}_0'], \text{~~~~~for each $A\subseteq \Omega$}
	\end{equation*}}
	\vis{Given an instance $\mathcal{I}_j$ where $j\in[m]$, let $P_j^{i,s}$ be the distribution of $r_i(s)$ under this instance. Then we have that $P_j = \prod_{i\in[m],s\in [L]} P_{j}^{i,s}$}.
	\arn{ Similarly given the problem instance $\mathcal{I}_0'$, let $P_0^{i,s}$ be the distribution of $r_i(s)$ under this instance. Then we have that $P_0 = \prod_{i\in[m],s\in [L]} P_{0}^{i,s}$}. 
	\arn{Let $S_{t} \subset [n]$ denote the set of arms discarded from memory till (and including) round $t$. For all $\omega \in \Omega$, let $T'_\omega = \arg\min_{t \leq T}\{t : S_t \neq \emptyset\}$ i.e. $T'_{\omega}$ is the first time-step since the beginning of the algorithm where some arm is discarded from memory. Let $A_1=\{\vis{\omega \in \Omega :} ~T'_\omega\leq L\}$ \vis{be the set of reward realizations for which $T'\leq L$}. \vis{Now fix some arm $i \in [m]$}. Define $A_2^{i}=\{\omega \in \Omega: i\in S_{T'_\omega}\}$ to be the event that the arm $i$ belongs to $S_{T'}$. Now, let $A^{i} = A_1 \cap A_2^{i}$ be the set of reward realizations such that $\forall \omega \in A^i$, $T'_\omega \leq L$ and arm $i$ is discarded from memory at $T'_\omega$}. 
	
\arn{(For now I am considering $A_1$ and $A^i$  as events. Later we can modify it )}

	\arn{For any deterministic algorithm of interest, we can assume that $\text{P}_0(A_1)\geq3/4$. If not, then such an algorithm would incur regret $\Omega(\frac{1}{m^2\cdot \epsilon^2})$ on the instance $\mathcal{I}_0'$. We now claim that there should exist an arm $i' \in [m]$ such that $P_0(A^{i'}) \geq \frac{3}{4m}$ otherwise $\text{P}_0(A_1)=\text{P}_0(\bigcup_{i\in[m]}A^i)\leq\sum_{i\in[m]}\text{P}_0(A^i)<3/4$} 
	
	Now apply Pinsker's inequality to the distributions $P_{0}$ and $P_{i'}$:
	%First, for each $\ell \in \{0,1,2,\ldots,m\}$, let us define the following probability distribution function on $\Omega$: $$P_{\ell,L}(A) = P_{\ell}[A ~|~ T' < L], \text{~~~~ for each $A \subseteq \Omega$}$$
	%Let $A' =\{\omega \in \Omega ~|~ i' \in S_{T'}\}$. 
	\begin{align*}
	2(P_{0}(A^{i'})-P_{i'}(A^{i'}))^2 \leq & KL(P_{0},P_{i'}) \tag{applying Pinsker's inequality}\\
	 = &\sum_{i\in[m]}\sum_{t=1}^{L} KL(P_0^{i,t},P_{i'}^{i,t}) \tag{using chain rule}\\
	 = & \sum_{i\in[m] \setminus \{i'\}} \sum_{t=1}^{L} KL(P_0^{i,t},P_{i'}^{i,t})\\
	& +\sum_{t=1}^{L} KL(P_0^{i',t},P_{i'}^{i',t}) \tag{Splitting the summation over arms}\\
	 \leq & ~0 + L\cdot 2\epsilon^2
	 \end{align*} 
	 \vis{In the last inequality, the first term of the summation is zero because, under instances $\mathcal{I}_0'$ and $\mathcal{I}_{i'}$, all arms $i\in[m], i \neq i'$ have identical reward distributions. To bound the second term in the summation, we use Theorem $2.5(d)$ from \cite{SLIVKINS2019}. We now have, }
	\begin{align*}
	P_0(A^{i'})- P_{i'}(A^{i'})&\leq \epsilon \sqrt{L} \\
	\Rightarrow P_{i'}(A^{i'}) &\geq P_0(A^{i'})-\epsilon \sqrt{L}\\
	&\geq \frac{3}{4m}-\frac{1}{2m} \tag{as $P_0(A^{i'})\geq \frac{3}{4m}$ and  $L=\frac{1}{4\cdot m^2\cdot \epsilon ^2}$}\\
	&= \frac{1}{4m}
	\end{align*}
	
	Now observe that $L = o(T)$. So $\forall \omega \in A^{i'}$ , the regret for instance $\mathcal{I}_{i'}^1$ is at least $\frac{\epsilon (T-T'_\omega)}{2}=\Omega(\epsilon T)$. 
	
	\arn{Now suppose that we choose an instance $\mathcal{I}$ uniformly at random from the family of $2m+1$ instances $\cup_{j=1}^m (\mathcal{I}_j^1 \cup \mathcal{I}_j^2)\cup\{\mathcal{I}_0'\}$. That is, we have $\mathbb{P}\big[\mathcal{I} = \mathcal{I}_{0}'\big]= \frac{1}{2m+1},\mathbb{P}\big[\mathcal{I} = \mathcal{I}_{j}^1\big]=\mathbb{P}\big[\mathcal{I} = \mathcal{I}_{j}^2\big] = \frac{1}{2m+1}$ for any $j \in [m]$.}  Then, 
	\begin{align*}
	&\mathbb{E}[R(T)]\\ &\geq  ~\mathbb{P}\big[\mathcal{I} = \mathcal{I}_{i'}^1\big]\cdot \mathbb{P}\Big[T'< L ~\big|~\mathcal{I}_{i'}\Big]\cdot P_{i'}(A^{i'})\cdot \Omega(\epsilon T)\\
	& ~~~+ \mathbb{P}\big[\mathcal{I} = \mathcal{I}_{i'}^2\big]\cdot \mathbb{P}\Big[T'\geq L ~\big|~\mathcal{I}_{i'}\Big] \cdot \Omega\Big(\frac{1}{m^2\cdot \epsilon ^2}\Big)	\\
	& = \frac{1}{4m^2}\cdot \mathbb{P}\Big[T'< L ~\big|~\mathcal{I}_{i'}\Big]\cdot \Omega\Big(\frac{T^{2/3}}{m^{1/3}}\Big) \\
	&~~~~+ \frac{1}{2m}\cdot \mathbb{P}\Big[T'\geq L ~\big|~\mathcal{I}_{i'}\Big]\cdot \Omega\Big(\frac{T^{2/3}}{m^{4/3}}\Big)\\
	& = ~\Big(\mathbb{P}\Big[T'< L ~\big|~\mathcal{I}_{i'}\Big] +\mathbb{P}\Big[T'\geq L ~\big|~\mathcal{I}_{i'}\Big]\Big)\cdot \Omega\Big(\frac{T^{2/3}}{m^{7/3}}\Big)\\
	&= ~\Omega\Big(\frac{T^{2/3}}{m^{7/3}}\Big)
	\end{align*}
	
	If $\epsilon = \frac{1}{m^{1/3}T^{1/3}}$, then $\mathbb{E}[R(T)]=\Omega\big(\frac{T^{2/3}}{m^{7/3}}\big)$, where the expectation is over that choice of input instance, randomness in reward and algorithm.
\end{proof}
\arn{We can modify the problem instances which we are considering such that if we are only storing at most $n/c$ arms where $c$ is a constant greater than 1, then under random arrival setting too $\mathbb{E}[R(T)]=\Omega\big(\frac{T^{2/3}}{m^{7/3}}\big)$ as for a particular instance, $(c-1)/c^2$ fraction of the total number of permutations incur huge regret.}


==> section_relatedWork.tex <==
\section{Related Work}
\label{section:related work}
The \MAB problem has been extensively studied in the literature and consequently a wide-variety of algorithms have been developed for both, the regret minimization problem as well as the best-arm identification problem. For the regret minimization problem, the UCB family of algorithms is well-studied in the literature. UCB-1 which was one of the earliest regret minimization algorithms proposed by \cite{AUER2002}, continues to be very popular due to its simplicity while providing a regret bound which only defers from the lower bound of \cite{LAI1985} in terms of problem-dependent constants. Thompson sampling has also shown to be optimal in the relatively recent work of \cite{AGRAWAL12}. For the best-arm identification problem, one of the earliest algorithm, called the Median-Elimination algorithm, was proposed by \cite{EVENDAR2002}. It is an $(\varepsilon,\delta)$-PAC algorithm with optimal sample complexity $O\big(\frac{n}{\varepsilon^2}\log(\frac{1}{\delta})\big)$. 

Crucially, all the algorithms mentioned above require the reward statistics of \emph{all} arms to be stored in the memory. With an increase in the number of arms, the memory requirement could become prohibitively large. Hence, an interesting new direction in the study of the \MAB problem is the design of algorithms with bounded arm memory. In particular, given $n$ arms, we would like to design an algorithm which, at any time, stores at most $m < n$ arms in memory. The maximum number of arms stored in memory at any instance of time is called the \emph{space complexity} of the algorithm.

%(the empirical means of)
%Majority of the literature on the stochastic \MAB problem can be divided into two parts based on the objective that an algorithm is trying to achieve. On the one hand is the literature that focuses on regret minimization in the \MAB problem \cite{BUBECK2012}, and on the other is the literature on \emph{best arm identification} in \MAB setting which is of interest in our work. In this variant, the goal of the decision-maker is to identify the best arm in terms of its true expected reward.

%The objective in this work is to establish PAC bounds on the expected reward of the arm output by the algorithm. More precisely, our goal is to provide an algorithm which outputs an $\varepsilon$-best arm with probability at least $1-\delta$ where $\varepsilon \in (0,1)$ and $\delta \in (0,1/2)$. Such an algorithm is called an $(\varepsilon,\delta)$-PAC algorithm. The work of \cite{EVENDAR2002} proposed the Median-Elimination algorithm which is a $(\varepsilon,\delta)$-PAC algorithm with optimal sample complexity which is $O\big(\frac{n}{\varepsilon^2}\log (\frac{1}{\delta})\big)$. Crucially, this algorithm (and its variants) require that the empirical mean of the rewards of \emph{each} arm be stored in memory so that the arms can be pulled in any time-step in the run of the algorithm which leads to a $O(n)$ \emph{space complexity}. Note that the space complexity only accounts for the number of arms that need to be stored in memory and not any other additional bits that might be needed to store the empirical means of each arm. Increasing the number of arms may lead to the space required by such an algorithm to be prohibitively large.

%The recent work by \cite{ASSADI2020} studies this variant of the best-arm identification problem. First, they propose an algorithm for the best-coin identification problem (equivalent to the \MAB problem with Bernoulli reward distributions), which stores exactly $1$ extra coin in memory at any time and has optimal sample complexity. They further extend their algorithm to the top-$k$ coins identification problem which stores $k$ coins in memory and has optimal sample complexity. Crucially though, both these algorithms assume that the gap parameter $\Delta$, which is the difference in the expected rewards of the best and the second-best coins, is known to the algorithm. 

%Finally, they propose an algorithm with space complexity $O(\log^* n)$ for the \SMAB problem where the gap parameter is not known to the algorithm. While their algorithm has optimal sample complexity, we prove via an adversarial input stream, that the algorithm is not $(\varepsilon, \delta)$-PAC as claimed (Claim 7.3 in the full version of \cite{ASSADI2020}).

%In the next section, we provide an adversarial input (a stream of arms) for the algorithm in Section 7 of \cite{ASSADI2020} and further show that Claim 7.3 in their work does not hold. In Section \ref{section:fix} we propose a fix to the algorithm which guarantees that the algorithm is $(\varepsilon,\delta)$-PAC with space complexity $O(\log^* n)$, while interestingly using a fewer number of arm pulls than the algorithm in \cite{ASSADI2020}.
%The work by \cite{CHAUDHURI2019} and \cite{LIAU2018} studies the \MAB problem with space constraints with the goal of minimizing the expected cumulative regret. The algorithms in both these works are multi-pass algorithms, i.e., they assume that an arm which has been discarded from memory can be read back into memory at a later time. \cite{LIAU2018} propose an upper-confidence bound based algorithm which achieves an expected cumulative regret bound of $O\big(\sum{i\neq i^*} \log(\frac{1}{\Delta_i})\frac{\log T}{\Delta_i}\big)$ which is within $\log(\frac{1}{\Delta_i})$ factor of the UCB-1 regret bound. Depending on the instance, the regret of this algorithm may be very high. \cite{CHAUDHURI2019} propose an algorithmic framework, which is given $m$ as input and that uses a \MAB algorithm as blackbox. When the \MAB algorithm used is UCB-1, their algorithm achieves expected regret of $O(nm + n^{3/2}m\sqrt{T \log(T/nm)})$.

